Federated Classification in Hyperbolic Spaces via Secure Aggregation of Convex Hulls

Hierarchical and tree-like data sets arise in many applications, including language processing, graph data mining, phylogeny and genomics. It is known that tree-like data cannot be embedded into Euclidean spaces of finite dimension with small distortion. This problem can be mitigated through the use of hyperbolic spaces. When such data also has to be processed in a distributed and privatized setting, it becomes necessary to work with new federated learning methods tailored to hyperbolic spaces. As an initial step towards the development of the field of federated learning in hyperbolic spaces, we propose the first known approach to federated classification in hyperbolic spaces. Our contributions are as follows. First, we develop distributed versions of convex SVM classifiers for Poincar\'e discs. In this setting, the information conveyed from clients to the global classifier are convex hulls of clusters present in individual client data. Second, to avoid label switching issues, we introduce a number-theoretic approach for label recovery based on the so-called integer $B_h$ sequences. Third, we compute the complexity of the convex hulls in hyperbolic spaces to assess the extent of data leakage; at the same time, in order to limit communication cost for the hulls, we propose a new quantization method for the Poincar\'e disc coupled with Reed-Solomon-like encoding. Fourth, at the server level, we introduce a new approach for aggregating convex hulls of the clients based on balanced graph partitioning. We test our method on a collection of diverse data sets, including hierarchical single-cell RNA-seq data from different patients distributed across different repositories that have stringent privacy constraints. The classification accuracy of our method is up to $\sim 11\%$ better than its Euclidean counterpart, demonstrating the importance of privacy-preserving learning in hyperbolic spaces.

==> algo_fl_secure.tex <==
% save the meaning of \AND and undefine it to keep algorithmic happy
\let\classAND\AND
\let\AND\relax
% load algorithmic
% save the new meaning of \AND and restore the one of the class
\let\algoAND\AND
\let\AND\classAND
% but when we start \begin{algorithmic} we want its own \AND
\AtBeginEnvironment{algorithmic}{\let\AND\algoAND}

\begin{algorithm}[htb]
  \caption{Secure Convex Hull Communication Algorithm}
  \label{alg:fl_secure}
  \begin{algorithmic}[1]
    \STATE \textbf{input:} Each client $l$ has vector $\boldsymbol{v}^{(l)}$ obtained from Section \ref{sec:labelencoding}.
    \STATE Each client $l\in [L]$ communicates $(S^{(l)}_1,\ldots,S^{(l)}_{2LK_{max}})$ to the server, where $K_{max}=\max_{i\in[L]}(|\hat{CH}_{+}^{(i)}|+|\hat{CH}_{-}^{(i)}|)$ and 
    $S^{(l)}_i=(\sum_{j\in [B]} v^{(l)}_j\cdot j^{i-1}+z^{(l)}_i) \text{ mod } q, i\in[2K_{max}L]$,  
     and $z^{(l)}_i$ is a random key uniformly distributed over $\mathbb{F}_p$ and hidden from the server. The keys $\{z^{(l)}_i\}_{l\in[L],i\in[2LK_{max}]}$ are generated offline using standard secure model aggregation so that $(\sum_{l\in[L]}z^{(l)}_i) \text{ mod } q = 0$.
    \STATE The server first computes the sum $S_i=(\sum_{l\in[L]}S^{(l)}_i) \text{ mod } q $. 
    Given $S_i$, the server computes the sum of labels $H_i=\sum_{l\in[L]}v^{(l)}_{i}$ for each bin index $i\in[B]$ as follows: Since there are at most $K_{max}L$ non-zero entries $H_i$, the server computes the polynomial $g(z)=\prod_{i:H_i\ne 0}(1-i\cdot z)$ using the Berlekamp-Massey algorithm \cite{Berlekamp1968AlgebraicCT,massey1969shift}. Then, the server factorizes $g(z)$ using the algorithm in \cite{kedlaya2011fast}, and finds the set $\{i:H_i\ne 0\}$. Finally, the server solves the linear equation set $S_i=\sum_{j:H_j\ne 0}H_j j^{i-1}$ for $i\in[2K_{max}L]$, by considering $H_j$ as unknown variables and $j^{i-1}$, 
 where $H_j\ne 0$, as known coefficients.
    \STATE Then, the server decodes the unique set of indices $i_1,\ldots,i_{h'}$, $h'\le h$ such that $H_i=a_{i_1}+\ldots+a_{i_{h'}}$, using brute force, which can be done since $a_1,\ldots,a_{2L}$ is a $B_h$ sequence. Finally, the server includes the bin centroid of the $i$th bin into $\hat{CH}_{-}^{(l)}$ and $\hat{CH}_{+}^{(l)}$ if $2l-1\in \{i_1,\ldots,i_{h'}\}$ and $2l\in \{i_1,\ldots,i_{h'}\}$, respectively. 
        \RETURN $\hat{CH}_{-}^{(l)}$, $\hat{CH}_{+}^{(l)}$, $l\in[L]$, reconstructed at the server.
  \end{algorithmic}
\end{algorithm}


==> algo_fl_svm.tex <==
% save the meaning of \AND and undefine it to keep algorithmic happy
\let\classAND\AND
\let\AND\relax
% load algorithmic
% save the new meaning of \AND and restore the one of the class
\let\algoAND\AND
\let\AND\classAND
% but when we start \begin{algorithmic} we want its own \AND
\AtBeginEnvironment{algorithmic}{\let\AND\algoAND}

\begin{algorithm}[H]
   \caption{Secure One-Shot Federated Hyperbolic SVM}
   \label{alg:fl_svm}
   \begin{algorithmic}[1]
    \STATE \textbf{Input:} Client data $(\bX^{(i)},\by^{(i)})$ for  $i\in[L]$; curvature constant $k$; Poincar\'e quantization parameters $\epsilon>0$ and $R< 1$; $B_h$ sequence.
    \STATE Each client $i\in[L]$ in parallel obtains $CH_{+}^{(i)}$ and $CH_{-}^{(i)}$, the sets of boundary points for Poincar\'e convex hulls of data points with local labels  $+1$ and $-1$ respectively.
    \STATE Each client $i\in[L]$ in parallel performs Poincar\'e bounded distance quantization (Appendix \ref{sec:disk_quantize_distance}) of points in $CH_{+}^{(i)}$ and $CH_{-}^{(i)}$, followed by another application of Poincar\'e convex hull algorithm to obtain the quantized boundary sets $\hat{CH}_{+}^{(i)}$ and $\hat{CH}_{-}^{(i)}$.
    \STATE Server recovers the quantized boundary sets $\{\hat{CH}_{+}^{(i)}\}_{i\in[L]}$ and $\{\hat{CH}_{-}^{(i)}\}_{i\in[L]}$ via the Secure Convex Hull Communication protocol (Alg. \ref{alg:fl_secure}).
    \STATE Server constructs a complete graph with $2L$ nodes, where each node represents one of $2L$ sets $\{\hat{CH}_{+}^{(1)},\ldots,\hat{CH}_{+}^{(L)},\hat{CH}_{-}^{(1)},\ldots,\hat{CH}_{+}^{(L)}\}$, and graph is partitioned into two groups with $L$ nodes each \ref{sec:graph_partition}. The two global clusters are arbitrarily assigned labels $+1$ and $-1$.   
    \STATE Server trains a hyperbolic SVM classifier (Section \ref{sec:back}) on the two labelled global clusters.
    \STATE\textbf{Return:} Server retains global reference point and SVM classifier.
\end{algorithmic}
\end{algorithm}
